Efficient Data Compression for 3D Sparse TPC via Bicephalous Convolutional Autoencoder

Real-time data collection and analysis in large experimental facilities present a great challenge across multiple domains, including high energy physics, nuclear physics, and cosmology. To address this, machine learning (ML)-based methods for real-time data compression have drawn significant attention. However, unlike natural image data, such as CIFAR and ImageNet that are relatively small-sized and continuous, scientific data often come in as three-dimensional data volumes at high rates with high sparsity (many zeros) and non-Gaussian value distribution. This makes direct application of popular ML compression methods, as well as conventional data compression methods, suboptimal. To address these obstacles, this work introduces a dual-head autoencoder to resolve sparsity and regression simultaneously, called \textit{Bicephalous Convolutional AutoEncoder} (BCAE). This method shows advantages both in compression fidelity and ratio compared to traditional data compression methods, such as MGARD, SZ, and ZFP. To achieve similar fidelity, the best performer among the traditional methods can reach only half the compression ratio of BCAE. Moreover, a thorough ablation study of the BCAE method shows that a dedicated segmentation decoder improves the reconstruction.

==> figures/NIU_cnnae_summary_.tex <==
% \documentclass[a4paper,10pt]{IEEEtran}
% \input{preamble}
% \input{figures/preamble_figure}

% \begin{document}
% \begin{figure*}[ht]

\begin{tikzpicture}
\def\scale{.5}
\tikzset{ myarrow/.style={{Latex[scale=\scale]}-{Latex[scale=\scale]}, color4, very thick} }
% ============================================ Encoder ======================================================
\node[mybox, rounded corners=10pt, draw=color4!80, fill=color1!40] (encoder) at (0, 0) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(.7,-1.9)}]$4\times$}] (Eb) at (0, 0) {\resblock{\scale}{90}{0}};
        \node[mybox, draw=color4, rotate=90, anchor=north, scale=.6] (El) at ([xshift=.1in]Eb.east) {$1\times1$ convolution};
        \draw[myarrow, shorten <=-.05in] (Eb) -- (El);
    \end{tikzpicture}
};
\node[fancytitle, right=5pt] (encoder_title) at ([yshift=.03in]encoder.north west) {Encoder $E$};
% =========================================================================================================== 

% ================================================== Decoders ==================================================  
\def\xs{.5in}
\def\ys{.65in}
\node[mybox, rounded corners=10pt, draw=color4!80, fill=color1!40, anchor=west] (decoder_c) at ([xshift=\xs, yshift=\ys]encoder.east) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(.7,-1.9)}]$3\times$}] (Dcb) at (0, 0) {\resblock{\scale}{90}{0}};
        \node[mybox, draw=color4, rotate=90, anchor=north, scale=.6] (Dcl) at ([xshift=.1in]Dcb.east) {transposed conv};
        \node[mybox, draw=color4, rotate=90, anchor=north, scale=.6, fill=color3] (Dcs) at ([xshift=0in]Dcl.south) {Sigmoid};
        \draw[myarrow, shorten <=-.05in] (Dcb) -- (Dcl);
    \end{tikzpicture}
};
\node[fancytitle, right=5pt] (decoder_c_title) at ([yshift=.03in]decoder_c.north west) {Clf.~Decoder $\dc$};
\node[mybox, rounded corners=10pt, draw=color4!80, fill=color1!40, anchor=west] (decoder_r) at ([xshift=\xs, yshift=-\ys]encoder.east) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(.7,-1.9)}]$3\times$}] (Drb) at (0, 0) {\resblock{\scale}{90}{0}};
        \node[mybox, draw=color4, rotate=90, anchor=north, scale=.6] (Drl) at ([xshift=.1in]Drb.east) {transposed conv};
        \draw[myarrow, shorten <=-.05in] (Drb) -- (Drl);
    \end{tikzpicture}
};
\node[fancytitle, right=5pt] (decoder_r_title) at ([yshift=.03in]decoder_r.north west) {Reg.~Decoder $\dr$};
\def\xss{.15in}
\draw[{Latex[scale=\scale]}-, very thick, color4] (encoder.east) -- ([xshift=\xss]encoder.east); 
\draw[-{Latex[scale=\scale]}, very thick, color4] ([xshift=\xss]encoder.east) 
	to [out=0,in=190] ([yshift=.08in]decoder_c.west);
\draw[-{Latex[scale=\scale]}, very thick, color4] ([xshift=\xss]encoder.east) 
	to [out=0,in=170] ([yshift=-.08in]decoder_r.west);
% ==============================================================================================================  

\node[mybox, draw=color5, fill=color5!40, anchor=south, align=center] (compressedData) at (encoder.south |- decoder_r.south west) {
    Compressed Data\\ 
    (float16)
};
\draw[-{Latex[scale=\scale]}, very thick, color4] (encoder.south) to [out=-90, in=90] (compressedData);

% ================================================== Loses ==================================================  
\node[mybox, fill=color3!80, draw=color4!80, anchor=north west, align=center, inner ysep=10pt] (loss_c) at ($(decoder_c.north west)!1.3!(decoder_c.north east)$) {
    Focal cross\\
    entropy\\
    \vspace*{-.2in}
};
\node[fancytitle, right=2pt] at (loss_c.north west) {Clf.~loss $\lc$};
\node[mybox, fill=color3!80, draw=color4!80, anchor=west, align=center, inner ysep=10pt] (loss_r) at ([yshift=-.08in]encoder -| loss_c.west) {
    Mean squared\\
    error\\
    \vspace*{-.2in}
};
\node[fancytitle, right=2pt] at (loss_r.north west) {Reg.~loss $\lr$};
\draw[myarrow] ($(decoder_c.north east)!(loss_c.west)!(decoder_c.south east)$) to (loss_c.west);
\draw[myarrow] ($(decoder_c.north east)!(loss_c.west)!(decoder_c.south east)$) to (loss_c.west);
\node[circle, draw=color4, fill=color4, very thick, inner sep=1pt, text=white, anchor=east] (plus) at ($(loss_r.east)!1.18!(loss_r.west)$) {\large $+$};
\draw[myarrow] ([yshift=-.08in]decoder_c.east) to[out=0,in=90] (plus);
\draw[myarrow] ([yshift=-.08in]decoder_r.east) to[out=0,in=-90] (plus);
\draw[myarrow] (plus) -- (loss_r);
% =========================================================================================================== 
\end{tikzpicture}

% \end{figure*}
% \end{document}

==> figures/TPC_full.tex <==
%\documentclass[usenames,svgnames,x11names,dvipnames,aspectratio=169]{beamer}
%
%\usepackage{amsmath,amssymb,amsthm,amsfonts,mathrsfs}
%% \usepackage[usenames,svgnames,x11names,dvipnames]{xcolor}
%
%\usepackage{tikz}
%\usetikzlibrary{shapes}
%
%\usepackage{pgfplots,pgfplotstable}
%\usepgfplotslibrary{groupplots}
%\pgfplotsset{compat=1.8}
%
%\begin{document}
%\begin{frame}
%\begin{figure}

\pgfmathsetmacro{\xdeg}{40}
\pgfmathsetmacro{\xx}{cos(\xdeg)}
\pgfmathsetmacro{\xy}{sin(\xdeg)}

\pgfmathsetmacro{\ydeg}{90}
\pgfmathsetmacro{\yx}{cos(\ydeg)}
\pgfmathsetmacro{\yy}{sin(\ydeg)}

\pgfmathsetmacro{\zdeg}{-20}
\pgfmathsetmacro{\zx}{cos(\zdeg)}
\pgfmathsetmacro{\zy}{sin(\zdeg)}

\newcommand{\tdcylInner}[5]{% origin x, origin y, origin z, radius, height
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}

    \filldraw[dashed, fill=cyan, fill opacity=0.2] (\height*\ct + #1, \height*\st + \y, \z) 
    	-- ++(0,0,\outerRadius) arc[start angle=\ang, delta angle=180, radius=\height] 
    	-- ++(0,0,-\outerRadius) arc[start angle=\ang+180, delta angle=180, radius=\height];
    \draw[dashed, ] (\height*\ct + #1, \height*\st + \y, \z + \outerRadius) arc[start angle=\ang, delta angle=-180, radius=\height];
    \filldraw[fill=cyan, fill opacity=0] (#1,\y,\z) circle[radius=\height];
}

\newcommand{\cylinder}[8]{
	% origin x, 
	% origin y, 
	% origin z, 
	% height, 
	% outer radius,
	% inner radius
	% color
	% opacity
	
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}
	
	% outer
    \filldraw[fill=#7, draw=#7, fill opacity=#8] 
    	(#1 + #5*\ct, #2 + #5*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=180, radius=#5] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=180, radius=#5];
    \draw[dashed, draw=#7] 
    	(#1 + #5*\ct, #2 + #5*\st, #3) 
    	arc[start angle=\ang, delta angle=-180, radius=#5];
    \draw[draw=#7] (#1 + #5*\ct, #2 + #5*\st, #3 + #4) 
    	arc[start angle=\ang, delta angle=180, radius=#5];
    % inner
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #6*\ct, #2 + #6*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=-180, radius=#6] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=-180, radius=#6];
    \draw[dashed, draw=#7] (#1 + #6*\ct, #2 + #6*\st, #3) 
    	arc[start angle=\ang, delta angle=180, radius=#6];
    \draw[draw=#7] (#1, #2, #3 + #4) circle[radius=#6]; 
}

\newcommand{\cylinderd}[8]{
	% origin x, 
	% origin y, 
	% origin z, 
	% height, 
	% outer radius,
	% inner radius
	% color
	% opacity
	
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}
	
	% outer
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #5*\ct, #2 + #5*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=180, radius=#5] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=180, radius=#5];
    \draw[dashed, draw=#7] 
    	(#1 + #5*\ct, #2 + #5*\st, #3) 
    	arc[start angle=\ang, delta angle=-180, radius=#5];
    \draw[draw=#7] (#1 + #5*\ct, #2 + #5*\st, #3 + #4) 
    	arc[start angle=\ang, delta angle=180, radius=#5];
    % inner
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #6*\ct, #2 + #6*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=-180, radius=#6] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=-180, radius=#6];
    \draw[dashed, draw=#7] (#1 + #6*\ct, #2 + #6*\st, #3) 
    	arc[start angle=\ang, delta angle=180, radius=#6];
    \draw[draw=#7] (#1, #2, #3 + #4) circle[radius=#6]; 
}


\begin{tikzpicture}[
	x={(\xx*1cm, \xy*1cm)},
	y={(\yx*1cm, \yy*1cm)},
	z={(\zx*1cm, \zy*1cm)},
]

    \path (1,0,0);
    \pgfgetlastxy{\xx}{\xy}
    \path (0,1,0);
    \pgfgetlastxy{\yx}{\yy}
    \path (0,0,1);
    \pgfgetlastxy{\zx}{\zy}
    
    \pgfmathsetmacro{\t}{(\zy * \yx - \zx * \yy)/ (\zy * \xx - \zx * \xy)}
    \pgfmathsetmacro{\ang}{atan(\t)}
    \pgfmathsetmacro{\c}{1/sqrt(1 + (\t)^2)}
    \pgfmathsetmacro{\s}{\t * \c}
    \pgfmathsetmacro{\angM}{atan(\t)-30}
    \pgfmathsetmacro{\cM}{sin(\angM)}
    \pgfmathsetmacro{\sM}{cos(\angM)}
    \pgfmathsetmacro{\angHM}{atan(\t)-45}
    \pgfmathsetmacro{\cHM}{sin(\angHM)}
    \pgfmathsetmacro{\sHM}{cos(\angHM)}
    \pgfmathsetmacro{\angTM}{atan(\t)-60}
    \pgfmathsetmacro{\cTM}{sin(\angTM)}
    \pgfmathsetmacro{\sTM}{cos(\angTM)}
    
	\pgfmathsetmacro{\x}{0}
	\pgfmathsetmacro{\y}{0}
	\pgfmathsetmacro{\z}{0}
	\pgfmathsetmacro{\height}{4}

	\pgfmathsetmacro{\core}{.85}
	\pgfmathsetmacro{\ld}{.45}
	\pgfmathsetmacro{\li}{\core + \ld}
	\pgfmathsetmacro{\lm}{\core + 2*\ld}
	\pgfmathsetmacro{\lo}{\core + 3*\ld}
	\pgfmathsetmacro{\op}{.4}
	
	\cylinder{\x}{\y}{\z}{\height}{\lo}{\lm}{Turquoise}{\op}
	\cylinderd{\x}{\y}{\z}{\height}{\lm}{\li}{SteelBlue}{\op}
	\cylinderd{\x}{\y}{\z}{\height}{\li}{\core}{DarkBlue}{\op}

		
	\draw[thick, Turquoise] (\x, \y, \z + \height) circle[radius=\lo];
	\draw[thick, SteelBlue] (\x, \y, \z + \height) circle[radius=\lm];
	\draw[thick, DarkBlue] (\x, \y, \z + \height) circle[radius=\li];
	
	\draw[dashed, thick, >=latex] (0, 0, 0) -- (0, 0, \height);
	\draw[->, thick, >=latex] (0, 0, \height) -- node[pos=1.1] {\large $z$} (0, 0, \height+.5*\height) ;
	
	\node[inner sep=0] (os) at (\x+\lo*\c, \y+\lo*\s, \z+\height) {};	
	\node[inner sep=0] (cs) at (\x+\core*\c, \y+\core*\s, \z+\height) {};
	\node[inner sep=0] (om) at (\x+\lo*\c, \y+\lo*\s, \z+1.08*\height) {};
	\node[inner sep=0] (mm) at (\x+\lm*\c, \y+\lm*\s, \z+1.08*\height) {};	
	\node[inner sep=0] (im) at (\x+\li*\c, \y+\li*\s, \z+1.08*\height) {};	
	\node[inner sep=0] (cm) at (\x+\core*\c, \y+\core*\s, \z+1.08*\height) {};
	\node[inner sep=0] (oe) at (\x+\lo*\c, \y+\lo*\s, \z+1.16*\height) {};	
	\node[inner sep=0] (ce) at (\x+\core*\c, \y+\core*\s, \z+1.16*\height) {};
	\draw[thick] (os) -- (oe);
	\draw[thick] (cs) -- (ce);
	\draw[->, thick, >=latex] (mm) -- (om);
	\draw[->, thick, >=latex] (im) -- (cm);
	\node[rotate=-20] at (\x+.75*\lo*\c, \y+.75*\lo*\s, \z+\height) {$48$ layers, $16$ each};
	% \draw[->, thick, black, >=latex] (om) -- node[midway, fill=white, rotate=-20, inner ysep=0, inner xsep=2, fill opacity=0, opacity=0, text opacity=1] {48} (cm);

\end{tikzpicture}
%\end{figure}
%
%\end{frame}
%\end{document}


==> figures/TPC_full_details.tex <==
%\documentclass[a4paper,10pt,onecolumn]{IEEEtran}
%\usepackage[utf8]{inputenc}
%\usepackage{amsmath,amssymb,amsthm,amsfonts,mathrsfs}
%\usepackage[usenames,svgnames,x11names,dvipnames]{xcolor}
%
%\usepackage{tikz}
%\usetikzlibrary{shapes}
%
%\usepackage{pgfplots,pgfplotstable}
%\usepgfplotslibrary{groupplots}
%\pgfplotsset{compat=1.8}
%
%\begin{document}
%\begin{figure}[ht]
%\centering
\pgfmathsetmacro{\xdeg}{40}
\pgfmathsetmacro{\xx}{cos(\xdeg)}
\pgfmathsetmacro{\xy}{sin(\xdeg)}

\pgfmathsetmacro{\ydeg}{90}
\pgfmathsetmacro{\yx}{cos(\ydeg)}
\pgfmathsetmacro{\yy}{sin(\ydeg)}

\pgfmathsetmacro{\zdeg}{-20}
\pgfmathsetmacro{\zx}{cos(\zdeg)}
\pgfmathsetmacro{\zy}{sin(\zdeg)}


\newcommand{\tdcylInner}[5]{% origin x, origin y, origin z, radius, height
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}

    \filldraw[dashed, fill=cyan, fill opacity=0.2] (\height*\ct + #1, \height*\st + \y, \z) 
    	-- ++(0,0,\outerRadius) arc[start angle=\ang, delta angle=180, radius=\height] 
    	-- ++(0,0,-\outerRadius) arc[start angle=\ang+180, delta angle=180, radius=\height];
    \draw[dashed, ] (\height*\ct + #1, \height*\st + \y, \z + \outerRadius) arc[start angle=\ang, delta angle=-180, radius=\height];
    \filldraw[fill=cyan, fill opacity=0] (#1,\y,\z) circle[radius=\height];
}

\newcommand{\cylinder}[8]{
	% origin x, 
	% origin y, 
	% origin z, 
	% height, 
	% outer radius,
	% inner radius
	% color
	% opacity
	
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}
	
	% outer
    \filldraw[fill=#7, draw=#7, fill opacity=#8] 
    	(#1 + #5*\ct, #2 + #5*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=180, radius=#5] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=180, radius=#5];
    \draw[dashed, draw=#7] 
    	(#1 + #5*\ct, #2 + #5*\st, #3) 
    	arc[start angle=\ang, delta angle=-180, radius=#5];
    \draw[draw=#7] (#1 + #5*\ct, #2 + #5*\st, #3 + #4) 
    	arc[start angle=\ang, delta angle=180, radius=#5];
    % inner
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #6*\ct, #2 + #6*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=-180, radius=#6] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=-180, radius=#6];
    \draw[dashed, draw=#7] (#1 + #6*\ct, #2 + #6*\st, #3) 
    	arc[start angle=\ang, delta angle=180, radius=#6];
    \draw[draw=#7] (#1, #2, #3 + #4) circle[radius=#6]; 
}

\newcommand{\cylinderd}[8]{
	% origin x, 
	% origin y, 
	% origin z, 
	% height, 
	% outer radius,
	% inner radius
	% color
	% opacity
	
    \path (1,0,0);
    \pgfgetlastxy{\cylxx}{\cylxy}
    \path (0,1,0);
    \pgfgetlastxy{\cylyx}{\cylyy}
    \path (0,0,1);
    \pgfgetlastxy{\cylzx}{\cylzy}
    
    \pgfmathsetmacro{\cylt}{(\cylzy * \cylyx - \cylzx * \cylyy)/ (\cylzy * \cylxx - \cylzx * \cylxy)}
    \pgfmathsetmacro{\ang}{atan(\cylt)}
    \pgfmathsetmacro{\ct}{1/sqrt(1 + (\cylt)^2)}
    \pgfmathsetmacro{\st}{\cylt * \ct}
	
	% outer
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #5*\ct, #2 + #5*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=180, radius=#5] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=180, radius=#5];
    \draw[dashed, draw=#7] 
    	(#1 + #5*\ct, #2 + #5*\st, #3) 
    	arc[start angle=\ang, delta angle=-180, radius=#5];
    \draw[draw=#7] (#1 + #5*\ct, #2 + #5*\st, #3 + #4) 
    	arc[start angle=\ang, delta angle=180, radius=#5];
    % inner
    \filldraw[dashed, draw=#7, fill=#7, fill opacity=#8] 
    	(#1 + #6*\ct, #2 + #6*\st, #3 + #4) -- ++(0, 0, -#4) 
    	arc[start angle=\ang, delta angle=-180, radius=#6] -- ++(0, 0, #4) 
    	arc[start angle=\ang+180, delta angle=-180, radius=#6];
    \draw[dashed, draw=#7] (#1 + #6*\ct, #2 + #6*\st, #3) 
    	arc[start angle=\ang, delta angle=180, radius=#6];
    \draw[draw=#7] (#1, #2, #3 + #4) circle[radius=#6]; 
}


\begin{tikzpicture}[
	x={(\xx*1cm, \xy*1cm)},
	y={(\yx*1cm, \yy*1cm)},
	z={(\zx*1cm, \zy*1cm)},
]

    \path (1,0,0);
    \pgfgetlastxy{\xx}{\xy}
    \path (0,1,0);
    \pgfgetlastxy{\yx}{\yy}
    \path (0,0,1);
    \pgfgetlastxy{\zx}{\zy}
    
    \pgfmathsetmacro{\t}{(\zy * \yx - \zx * \yy)/ (\zy * \xx - \zx * \xy)}
    \pgfmathsetmacro{\ang}{atan(\t)}
    \pgfmathsetmacro{\c}{1/sqrt(1 + (\t)^2)}
    \pgfmathsetmacro{\s}{\t * \c}
    \pgfmathsetmacro{\angM}{atan(\t)-30}
    \pgfmathsetmacro{\cM}{sin(\angM)}
    \pgfmathsetmacro{\sM}{cos(\angM)}
    \pgfmathsetmacro{\angHM}{atan(\t)-45}
    \pgfmathsetmacro{\cHM}{sin(\angHM)}
    \pgfmathsetmacro{\sHM}{cos(\angHM)}
    \pgfmathsetmacro{\angTM}{atan(\t)-60}
    \pgfmathsetmacro{\cTM}{sin(\angTM)}
    \pgfmathsetmacro{\sTM}{cos(\angTM)}
    
%    \pgfmathsetmacro{\angP}{atan(\t)+30}
%    \pgfmathsetmacro{\cP}{sin(\angP)}
%    \pgfmathsetmacro{\sP}{cos(\angP)}

	\pgfmathsetmacro{\x}{0}
	\pgfmathsetmacro{\y}{0}
	\pgfmathsetmacro{\z}{0}
	\pgfmathsetmacro{\height}{4}

	\pgfmathsetmacro{\core}{.85}
	\pgfmathsetmacro{\ld}{.45}
	\pgfmathsetmacro{\li}{\core + \ld}
	\pgfmathsetmacro{\lm}{\core + 2*\ld}
	\pgfmathsetmacro{\lo}{\core + 3*\ld}
	\pgfmathsetmacro{\op}{.4}
	
	\cylinder{\x}{\y}{\z}{\height}{\lo}{\lm}{Turquoise}{\op}
	\cylinder{\x}{\y}{\z + \height}{\height}{\lm}{\li}{SteelBlue}{\op}
	\cylinder{\x}{\y}{\z + 2*\height}{\height}{\li}{\core}{DarkBlue}{\op}
	\draw[thick, Turquoise] (\x, \y, \z + \height) circle[radius=\lo];
	\draw[thick, SteelBlue] (\x, \y, \z + \height + \height) circle[radius=\lm];
	\draw[thick, DarkBlue] (\x, \y, \z + \height + 2*\height) circle[radius=\li];
	\node[fill=LightBlue, fill opacity=0, text opacity=1, rotate=10, inner ysep=0, inner xsep=2] at (\x+\lo*\cM, \y+.2+\lo*\sM, \z+\height) {$2304$ colums};
	\node[fill=LightBlue, fill opacity=0, text opacity=1, rotate=10, inner ysep=0, inner xsep=2] at (\x+\lm*\cM, \y+.2+\lm*\sM, \z+\height + \height) {$1536$ columns};
	\node[fill=LightBlue, fill opacity=0, text opacity=1, rotate=10, inner ysep=0, inner xsep=2] at (\x+\li*\cM, \y+.2+\li*\sM, \z+\height + 2*\height) {$1152$ columns};
	
	\node[inner sep=0] (a) at (\x-\lo*\c, \y-\lo*\s, \z) {};
	\node[inner sep=0] (ad) at (\x-\lo*\c-.2*\lo*\c, \y-\lo*\s-.2*\lo*\s, \z) {};
	\node[inner sep=0] (am) at (\x-\lo*\c-.1*\lo*\c, \y-\lo*\s-.1*\lo*\s, \z) {};
	
	\node[inner sep=0] (b) at (\x-\lo*\c, \y-\lo*\s, \z+\height) {};
	\node[inner sep=0] (bd) at (\x-\lo*\c-.2*\lo*\c, \y-\lo*\s-.2*\lo*\s, \z+\height) {};
	\node[inner sep=0] (bm) at (\x-\lo*\c-.1*\lo*\c, \y-\lo*\s-.1*\lo*\s, \z+\height) {};
	
	\draw[thick, black] (a) -- (ad);	
	\draw[thick, black] (b) -- (bd);
	\draw[<->, thick, black, >=latex] (am) -- node[midway, fill=white, rotate=-20, inner ysep=0, inner xsep=2] {$498$ rows} (bm);


\end{tikzpicture}
%\end{figure}
%\end{document}


==> figures/cnnae_summary.tex <==
% \documentclass[a4paper,10pt]{IEEEtran}
% \input{../preamble}
% \input{figures/preamble_figure}
% \usetikzlibrary{shapes.geometric, arrows}

% \begin{document}
% \begin{figure}[ht]
% \centering

\begin{tikzpicture}[scale=\summaryScale, every node/.style={scale=\summaryScale}]

\tikzstyle{trap} = [
    trapezium, 
    trapezium left angle=80, 
    trapezium right angle=80, 
	draw=color4!80, 
	fill=color1!40, 
	very thick,
    rounded corners, 
    inner xsep=2pt, 
    inner ysep=0pt,
    align=center,
    inner xsep=0pt,
    inner ysep=5pt,
    %align=right, 
    text width=.148\textwidth, % curious thing, has to be adjust manually for the content to stay in middle
    % minimum width=3cm, %!!!!!! jiu shi ni! po huai fen zi!
]

\def\scale{.5}
\tikzset{ myarrow/.style={-{Latex[scale=\scale]}, color4, very thick} }
\node[trap,rotate=-90,] (encoder) at (0, 0) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(.9, -.4)}, rotate=90]$4\times$}] (Eb) at (0, 0) {\resblock{\scale}{180}{0}};
        \node[mybox, draw=color4, anchor=south, scale=.75, rotate=180] (El) at ([xshift=0in, yshift=.3in]Eb.north) {$1\times1\times1$ Conv};
        \draw[myarrow] (Eb) -- (El);
    \end{tikzpicture}
};
\node[fancytitle, right=5pt, rotate=-10] (encoder_title) at ([xshift=.05in, yshift=.1in]encoder.south west) {Encoder $E$};
\node[mybox, draw=color5, fill=color5!40, anchor=south, align=center, rotate=90] (compressedData) at ([xshift=.4in]encoder.north) {Compressed Data};
\draw[myarrow] (encoder) -- (compressedData);


\def\xs{.75in}
\def\ys{.65in}
\node[trap,rotate=100, anchor=north] (decoder_c) at ([xshift=\xs, yshift=\ys]encoder.north) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(-1, -2.1)}, rotate=-90]$3\times$}] (Dcb) at (0, 0) {\resblock{\scale}{0}{0}};
        \node[mybox, anchor=north, scale=.75, draw=color4] (Dcl) at ([xshift=0in, yshift=-.15in]Dcb.south) {deConv};
        \node[mybox, anchor=north, scale=.75, draw=color4, fill=color3] (Dcs) at ([xshift=0in]Dcl.south) {Sigmoid};
        \draw[myarrow] (Dcb) -- (Dcl);
    \end{tikzpicture}
};
\node[fancytitle, rotate=20, anchor=west] (decoder_c_title) at ([xshift=-.1in, yshift=-.05in]decoder_c.north east) {Seg.~Decoder $\ds$};
\node[trap,rotate=80, anchor=north] (decoder_r) at ([xshift=\xs, yshift=-\ys]encoder.north) {
    \begin{tikzpicture}
        \node[inner sep=0pt, label={[shift={(-1, -2.1)}, rotate=-90]$3\times$}] (Drb) at (0, 0) {\resblock{\scale}{0}{0}};
        \node[mybox, anchor=north, scale=.75, draw=color4] (Drl) at ([xshift=0in, yshift=-.15in]Dcb.south) {deConv};
        \draw[myarrow] (Drb) -- (Drl);
    \end{tikzpicture}
};
\node[fancytitle, right=5pt, anchor=west] (decoder_r_title) at ([xshift=-.1in]decoder_r.north east) {Reg.~Decoder $\dr$};
\def\xss{.45in}
\draw[color4, very thick] (compressedData.south) -- ([xshift=\xss]encoder.north); 
\draw[myarrow] ([xshift=\xss]encoder.north) to [out=0,in=190] ([yshift=.08in]decoder_c.north);
\draw[myarrow] ([xshift=\xss]encoder.north) to [out=0,in=170] ([yshift=-.08in]decoder_r.north);

% ================================================== Loses ==================================================  
\node[mybox, fill=color3!80, draw=color4!80, anchor=west, align=center, inner ysep=10pt] (loss_c) at ([xshift=.5in]decoder_c.south) {
    Focal cross\\
    entropy\\
    \vspace*{-.2in}
};
\node[fancytitle, right=2pt] at (loss_c.north west) {Seg.~loss $\ls$};
\node[mybox, fill=color3!80, draw=color4!80, anchor=west, align=center, inner ysep=10pt] (loss_r) at ([yshift=-.08in]encoder -| loss_c.west) {
    Mean squared\\
    error\\
    \vspace*{-.2in}
};
\node[fancytitle, right=2pt] at (loss_r.north west) {Reg.~loss $\lr$};

\draw[myarrow] (decoder_c.south) to (loss_c.west);
\node[circle, draw=color4, fill=color4, very thick, inner sep=1pt, text=white, anchor=east] (plus) at ($(loss_r.east)!1.1!(loss_r.west)$) {\large $\times$};
\draw[myarrow] ([yshift=-.1in]decoder_c.south) to[out=0,in=90] (plus);
\draw[myarrow] (decoder_r.south) to[out=0,in=-90] (plus);
\draw[myarrow] (plus) -- (loss_r);
% =========================================================================================================== 


\end{tikzpicture}

% \end{figure}
% \end{document}
